Active Classification of Moving Targets with Learned Control Policies

In this paper, we consider the problem where a drone has to collect semantic information to classify multiple moving targets. In particular, we address the challenge of computing control inputs that move the drone to informative viewpoints, position and orientation, when the information is extracted using a "black-box" classifier, e.g., a deep learning neural network. These algorithms typically lack of analytical relationships between the viewpoints and their associated outputs, preventing their use in information-gathering schemes. To fill this gap, we propose a novel attention-based architecture, trained via Reinforcement Learning (RL), that outputs the next viewpoint for the drone favoring the acquisition of evidence from as many unclassified targets as possible while reasoning about their movement, orientation, and occlusions. Then, we use a low-level MPC controller to move the drone to the desired viewpoint taking into account its actual dynamics. We show that our approach not only outperforms a variety of baselines but also generalizes to scenarios unseen during training. Additionally, we show that the network scales to large numbers of targets and generalizes well to different movement dynamics of the targets.

==> backup/preCoRL_results_backup.tex <==
\begin{figure}[!t] 
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.32\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/ntracked_sf_goal.png}
        \caption{\footnotesize{Static targets.}\label{fig:static200}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.32\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/unclass_histogram_sf_goal.png}
        \caption{\footnotesize{Constant velocity.}\label{fig:ctevel200}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.32\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/class_percentage_sf_goal.png}
        \caption{\footnotesize{Social forces.}\label{fig:sfgoal200}}
        \end{subfigure}
        % \hfill

        
        \caption{\footnotesize{Comparison of our policy with the baselines in environments containing up to 50 targets with different dynamics.}} \label{fig:firstperformance}
\end{figure}

% \begin{figure}[!t] 
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{images/performance_scale/unclass_histogram_static.png}
%         \caption{Static targets.\label{fig:static200}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{images/performance_scale/unclass_histogram_cte_vel.png}
%         \caption{Constant velocity.\label{fig:ctevel200}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{images/performance_scale/unclass_histogram_sf_goal.png}
%         \caption{Social forces.\label{fig:sfgoal200}}
%         \end{subfigure}
%         % \hfill
        
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{images/performance_scale/class_percentage_static.png}
%         \caption{Static targets.\label{fig:static200}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{images/performance_scale/class_percentage_cte_vel.png}
%         \caption{Constant velocity.\label{fig:ctevel200}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{images/performance_scale/class_percentage_sf_goal.png}
%         \caption{Social forces.\label{fig:sfgoal200}}
%         \end{subfigure}
%         % \hfill
        
%         \caption{Comparison of our policy with the baselines along an episode in environments of 16 targets. a)-c) Plots the number unclassified targets simultaneously observed at each time step for each environment dynamics. The monotonically increasing plots in d)-f) represent the percentage of classified targets along the episode for each method.} \label{fig:singleEpisodeperformance}
% \end{figure}

\section{Results}
In this section, we provide a thorough evaluation of the trained policy and analyze its robustness and scalability properties in comparison with other baselines.

\subsection{Performance evaluation}
We evaluate the performance of our method in environments presenting different amount of targets and different target dynamics: static, constant velocity and social forces dynamics. Social forces pedestrian dynamics are modeled after~\citep{socialforces}. The idea of the latter is to test the robustness of our method in environments where the targets show a different behavior than the one seen in training. Each policy is given a timeout of $T=200$ time steps and is evaluated by the percentage of targets it is able to classify before the end of the episode. 

The baselines used for comparison are:
\begin{itemize}    
    \item \textbf{Hand-crafted}: hard-coded policy that, given a target's information, guides the drone to the position 2m in front of it, pointing the camera at it.
    
    \item \textbf{Single-target}: A learned policy that, given the observation of one target, has been trained to classify it as fast as possible.
\end{itemize}

The Single-target policy's training conditions are almost identical to our method, the only difference being end of the episode when the selected target is classified.
%Instead of following the same training schedule, it has been trained to convergence in single-target scenarios.

Since the two baselines are designed to classify one target at a time, the extension to multiple targets is done by sequential classification of them. Unclassified targets are ordered by their distance to the drone. Once a target has been selected the drone must classify it before choosing another one. Observations of targets other than the chosen one are still accounted for the information fusion and belief computation.

We evaluate the three methods for 50 episodes in environments with 1 to 50 targets and the three dynamics, to evaluate them in both in-training and out-of-training scenarios. For the sake of fairness, we randomly sample the initial configuration for each combination of target quantity and dynamics, save it, and evaluate each policy under the same random initial conditions. We have also trained and evaluated each learned policy with three different seeds. The shown results are the mean and standard deviations of the average results obtained for all three of them across all episodes.


In Fig.~\ref{fig:firstperformance} we report the percentage of targets that each method has been able to classify in every setting. In general, as expected, there is a drop in the percentage of targets that can be classified when their quantity and density increases. This is due to the fact that the task takes theoretically longer to complete and the number of occlusions among targets increases. This becomes even more apparent in static environments, where targets might be completely occluded by other targets or directly facing into a wall, making it more difficult, or even impossible, to classify them.

While our method behaves similarly to the learned baseline when targets are static, it clearly outperforms both baselines in dynamic environments. It not only performs well in scenarios seen during training, but it also manages to scale well and better to scenarios where the number and density of targets to classify is much greater than seen during training ($>$12 targets). 

We also monitor the evolution of the number of unclassified targets along the episode in scenarios with 16 targets (fig. \ref{fig:singleEpisodeperformance} a)-c)). During the first half of the episode, our method consistently is shown to observe and provide classification estimates of more targets than the baselines at every time step. Then, as targets get classified along the episode (as seen in d)-f)), the pool of unclassified ones grows smaller and their viewpoints become sparsely distributed across the environment. This is the reason why the number of unclassified targets that can be observed simultaneously with minimal time step and movement cost drops significantly.

Our architecture is able to account for all targets' available information at the same time. This means that it is able to learn strategies that are likely to prioritise to go towards viewpoints allowing simultaneous observations of multiple unclassified targets.%, even if that means losing classification accuracy for some of them. 
Additionally, the baselines are bound to classify the targets following a heuristic proximity-based priority order. This order of priority might not be the best one, as it should depend on the relative pose and velocity of the targets with respect to the camera and the classifier sensor model. However, we do not have access to the latter and both baselines cannot reason about all targets' information at the same time, which is why these results show that, at least, our method is able to learn a better classification priority order.

It is also remarkable to see that the method is able to generalize and perform well when the targets follow other dynamics than seen during training. This is probably due to the fact that targets under social forces behave similarly to their constant velocity counterpart when traveling to their goals. Also, due to the repulsive force of dynamic and static obstacles (targets and walls), it is not likely for two targets to be facing each other or against a wall. This makes it easier for our method to find suboptimal viewpoints allowing to obtain good classification estimates of multiple targets at a time. In contrast, the learned baseline is not robust to this change in dynamics as it cannot learn to avoid target occlusions.

In Fig.~\ref{fig:horizonanalysis}, we provide results on the baselines and our method's performance under different timeout conditions in scenarios with 16 targets with constant velocity dynamics. It shows empirical proof that our method is able to complete the task if given enough time. Also, we show that our proposed method is able to approach the end of the task generally faster than the baselines. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=8.5cm]{images/horizon/horizon_analysiscte_vel.png}
%     \caption{\footnotesize{Performance for 16 targets following constant velocity dynamics when the length of an episode (timeout) is varied. Note that all methods classify all targets eventually, but that our approach is much faster.}
%     %Timeout analysis in scenarios of 16 targets following constant velocity dynamics.
%     }
%     \label{fig:horizonanalysis}
% \end{figure}

\subsection{Ablations}
Next we compare the performance of our method with that of ablated architectures. While there are architectures in the learning-based motion planning literature that map environment representations of an arbitrary dimension to a latent representation vector of fixed dimension, these methods are either not permutation invariant~\citep{meverett2021}, or weight each element in the input sequence equally~\citep{Hsu2021}. We argue that these are important biases that must be encoded into our architecture for it to be more robust and consistent. Inspired by these two works, we design ablated versions of our architecture that mirror the architectural choices in these two works and train them following the same training schedule we use for our method:
\begin{itemize}    
    \item \textbf{LSTM encoder}~\citep{meverett2021}: The self-attention and attention pooling layers are substituted by a linear layer followed by an LSTM. Every unclassified target is inversely sorted by proximity to the drone. The first layer encodes each target's information, and the sequence is fed into the LSTM. 
    
    
    \item \textbf{DeepSets decoder}~\citep{Hsu2021}: It follows the architecture as in our method but we replace the $PMA_1$ layer by a mean pooling layer. 
\end{itemize}

In Fig. \ref{fig:ablations}, we show how these ablations scale and generalize to scenarios not seen during training, having an increasing amount of targets following social forces dynamics. While both ablations show good performance, our architecture choice outperforms both of them, showing better scalability properties in scenarios that none of the policies have seen before.

% \begin{figure}[t] % MUST BE UPDATED
%     \centering
%     \includegraphics[width=0.95\linewidth]{images/ablations/ntracked.png}
%     \caption{\footnotesize{Comparison of our method with ablations.}}
%     \label{fig:ablations}
% \end{figure}

The LSTM encoder requires for each element in a sequence to be fed sequentially. This results in retaining more information about the last input elements than the first ones, requiring to feed high-priority targets later in the sequence. Learning-based methods in safe navigation can use proximity to estimate target priority. However, in the classification problem there might be far away targets that are easier to classify depending on the orientation and visibility conditions.
The DeepSets decoder ablation does not impose any order on the sequence, and aggregates their latent representations with equal weight. Nevertheless, there are targets that should weight more than others when deciding on the future action. For instance, unclassified or occluded targets should have more weight in guiding the drone's actions than already classified targets not occluding the observation of others.

\section{Experimental Results}


==> sec/additional_content/POMDP_formulation.tex <==
%\subsection{Reinforcement Learning}\label{sec:appendixA}
\section{POMDP Formulation}
%We formulate a reinforcement learning problem to compute an efficient active classification control policy. By considering pre-trained classifiers with fixed parameters being used as sensors, and target dynamics and belief updates as part of the transition function, this problem can be transformed into a POMDP~\cite{KAELBLING199899}. The POMDP is composed of six components, including state space, action space, observation space, transition model, observation model and reward function.
%\subsection{State space $S$}
%The state space accounts for the current physical state of the environment ($\vx_t,\vy_t$), the real classes of each target ($\vb^*$) and the current drone beliefs (${\vb}_t$). Therefore, the state at time $t$ can be defined as:

% \begin{equation}
%     \vs_t := [\vx_t,\vy_t, \vb^*, {\vb}_t] \in \cS
% \end{equation}

%\subsection{Observation Space $Z$}
%The main purpose is to guide the camera towards informative locations at the right time, which is why we consider all the relative target poses available. This is not unrealistic, as there are already available methods to provide information on target states~\cite{sung2017}.

%The available information for the drone is its current updated belief on each target $j$'s classes, and the current output from the sensor. 
%Additionally, we consider Boolean variables, $l^j_t$ to describe targets that have already been classified within an arbitrary quality threshold, $b_{max}$, 
% \begin{equation}
%     l^j_t = 
%     \begin{cases}
%       1 & \hbox{if }\max_{c\in C}b_c^j \geq b_{max}\\
%       0 & \hbox{otherwise}\\
%       \end{cases}.
% \end{equation}
% Therefore, the observation over a target is described by:
% \begin{equation}
%     \vo^j_t = [\tilde{\vy}^j_t, \mathcal{H}[\vect{p}^j_t], \mathcal{H}[\vb^j_t], l^j_t]
% \end{equation}
% The joint observation over all targets is described by $\vo_t=\{\vo^j_t|\forall j\in\cJ\}$.

%\newcont{Note that we only require the entropy of the beliefs ($\mathcal{H}[\vb^j_t]$) and measurements ($\mathcal{H}[\vect{p}^j_t]$), which allows our method to handle an arbitrary number of classes $C$. }

\subsection{Action Space $\cA$}
Every time step, the drone leverages the information it has available and chooses the next viewpoint in its neighborhood to move towards, expressed in terms of its camera local reference frame. In practice, this translates into choosing:
\begin{equation}
\begin{split}
    \va_t := [\Delta q_{x',t}, \Delta q_{y',t}, \Delta\psi_{t}]\\
\end{split}
\end{equation}
where $x',y'$ represent the $x$ and $y$-axis in the camera's local reference, and $\Delta q_{i,t}$, $\forall i\in\{x',y'\}$ are confined to a neighborhood of the current drone's pose: $\Delta q_{x',t},\Delta q_{y',t}\in[-\Delta q^{max},\Delta q^{max}]$, where $\Delta q^{max}$ denotes the maximum distance along each local axis that the drone can reach within one second at constant velocity. This also applies for the camera heading $\psi^0$. 

% Having chosen a new viewpoint, the drone drives towards it at constant speed for $\tau_h$ seconds:

% \begin{equation}
% \begin{split}
%     \vq_{t+1}^0 & := \vq_{t}^0 +\tau_h\hbox{Rot}(\psi_t^0)[\Delta q_{x',t}, \Delta q_{y',t}]^T\\
%     \psi_{t+1}^0 & := \psi_t^0+\tau_h\Delta\psi_{t}\\
% \end{split},
% \end{equation}
% where $\hbox{Rot}(\psi_t^0)\in SO(2)$ is the rotation matrix that maps the camera's reference frame to the global reference frame. At test time we use a low-level control policy to guide the drone towards the defined new position and orientation. In Section \ref{sec:policy_network}, we detail how viewpoint recommendations are obtained and tracked through receding horizon optimal control at test time.

%\subsection{Reward $R(\vs_t,\va_t)$}
%The reward function is chosen based on the multiple behaviors we want to achieve. It aims for the learned control policy to move to informative viewpoints that will allow the drone to classify as many targets as possible while being time and energetically efficient. The reward value $R(\vs_t,\va_t)$ is the immediate reward the drone gets at state $\vs_t$ after applying action $\va_t$, and is composed by the combination of different reward terms. 

% First, the drone is rewarded for the completion of the task to motivate the classification of all targets if possible,
% \begin{equation}\label{rew:taskcompletion}
% R_{AC}(\vs_t) = 
% \begin{cases}
%       w_{AC} & \hbox{if }l^j_{t} = 1,~\forall j\in\cJ\\
%       0 & \hbox{otherwise}\\
%      \end{cases}
% \end{equation}

% The second reward encourages to classify every target. It accounts for the fact that, even if the drone does not manage to complete the task, it still needs to fully classify as many targets as possible,
% \begin{equation}\label{rew:targetclass}
% R_{class}(\vs_t) = w_{class}\sum^{M}_{j=1}(l^j_{t}-l^j_{t-1})
% \end{equation}

% The third reward comes directly from the problem formulation. It encourages to quickly gain information on the targets' class. Information gain is modelled by how much the entropy of the beliefs has decreased due to the new information gathered at time step $t$. Therefore, this dense reward encourages to simultaneously observe, if possible, multiple unclassified targets,
% \begin{equation}\label{rew:entropydecrease}
% \begin{split}
% R_{ent}(\vs_t) = w_{ent}\sum^{M}_{j=1}\mathcal{H}(\vb^j_{t-1})-\mathcal{H}(\vb^j_{t})
% \end{split}
% \end{equation}


% The fourth reward encourages to finish the task as quickly as possible, and is defined by a constant penalty term per time step,
% \begin{equation}\label{rew:timepunishment}
% R_{time} = w_{time}
% \end{equation}

% The last reward acts as a regularization term to limit energy consumption and oscillating behaviors by penalizing the magnitude of action $a_t$,
% \begin{equation}\label{rew:energycompt}
% R_{m}(\va_t) = w_{m}(\sqrt{\Delta q_{x',t}^2 + \Delta q_{y',t}^2} + |\Delta\psi_{t}|)
% \end{equation}

% $w_{AC}$, $w_{class}$, $w_{ent}$, $w_{time}$, $w_{m}$ are weights that scale each term appropriately.
% Summing up, these terms are combined in a weighted sum,
% \begin{equation}\label{rew:fullrew_appendix}
% \begin{split}
%     R(\vs_t,\va_t) = & R_{AC}(\vs_t) + R_{class}(\vs_t) +R_{ent}(\vs_t) - R_{time}- R_{m}(\va_t),
% \end{split}
% \end{equation}

% The observation model ($\cO$) depends on the state of the system and the drone sensor model $h$, whereas the transition model ($\cT$) depends on the target and drone dynamics, the drone sensor models and how the belief updates are computed, discussed in the next subsection.

==> sec/backup/SimuObs.tex <==
\section{Realistic Results} \ref{ref:relResults}

% \subsection{Observation Model}
% To ascertain our framework's sim-to-real capabilities, we test its performance in an environment generated with Unreal Engine using AirSim to simulate drone control and perception. We use open-source 3D human meshes, produced in \textit{MakeHuman} \cite{makehuman}, to simulate our targets in Unreal Engine, which move to random goals in the environment while avoiding collisions. To remain close to the use-case shown in the earlier simpler environment, pedestrian classes are represented by a painted number in the front of their t-shirt. We avoid the problem of data association by using AirSim API, which allows us to obtain the cropped image of every pedestrian in the drone's field of view (FOV). To map these images to their respective class probability distribution, an implementation of YoloV3 algorithm is used to detect and classify digits. We train the algorithm using a dataset of rotated, up-scaled and down-scaled MNIST images shown in Fig. \ref{fig:mnist_dataset}. 

% The output of the algorithm consists in a set of bounding boxes, each one associated to a detected digit and a normalized score stating how sure the algorithm is of it's detection. We rule out those boxes which area is smaller than a threshold $B_a$ and take the box with the highest score. If the detected digit is correct, we use its score as the target class probability estimate, distributing the remaining probability mass among the other classes. We assume there is an oracle that allows us to detect when the sensor has not captured useful information (e.g. no detection, incorrect digit, or lower score than uniform distribution), at which point we output a uniform probability distribution. The use of this oracle could be relaxed by using epistemic uncertainty-aware models to perform detect and classify (e.g. Gaussian Processes, Deep Bayesian Networks) but it is out of scope of this paper. Note that under no circumstances our framework has any knowledge of the classification algorithm.

% To avoid the computational cost of using AirSim and YoloV3 during training, the training environment explained in Section \ref{sec:implementation} is enhanced with approximated real perception. We use AirSim to extract a dense library of pedestrian observations of all classes in different relative poses from the drone's FOV. For each class, each pose-dependent image is used to compute and save a probability distribution using the aforementioned method. During training, for each target in the drone's FOV, we use the probability distribution of library image whose pose is the closest to the current target relative pose to the camera.


%each target in the drone's FOV is associated to the output probability distribution whose re 
 
%to it's class closest pose in the library

%the probability distribution obtained from the library whose pose is the closest 

%The set of probability distributions for each class are saved 

%Training in AirSim takes a prohibitive amount of time. To bypass this limitation, we enhance our current training envrionment with approximated real perception. We 


%If there is no detection, the detected digit is incorrect, or correct but with a score below uniform probability, then we assume the sensor has not captured any kind of useful information and output a uniform probability distribution. 

%Apart from this, note that under no circumstances our framework has any knowledge of the classification algorithm's model.


%use an actual black-box classification algorithm which requires its use during training as well. We 
%The next step is to test this framework in a realistic environment and an actual

%Points to explain:

%- We want to test in realistic environment such as AirSim
%- This requires to use the perception model while training
%- We train an implementation of YoloV3 to detect and classify MNIST numbers in an image using a dataset of MNIST numbers rotated and/or up/downscaled.

%Training time:
%- Training in AirSim takes a prohibitive amount of time
%- To simulate the same perception during training we generate a library of human poses inside the FOV(explain the library)
%- We then compute the probability estimates for each image in the library and store them.
%- During training, for each target in the FOV we obtain the proba estimate of the library image that is closest to the current position.

%Test time:
%During test time, we get the cropped image from every target in the FOV from AirSim and do the same process as before.





% \begin{figure}[t!] 
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.10\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class1/-100.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{-100$^o$}\label{fig:-100}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.10\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class1/-140.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{-140$^o$}\label{fig:-140}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.10\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class1/-180.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{$\pm$180$^o$}\label{fig:-180}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.13\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class1/140.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{140$^o$}\label{fig:140}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \caption{\footnotesize{Probability heat-map of the employed black-box classifier for a target of class 1. For a robot placed at the bottom, facing upwards and a FOV of $90^o$, every plot shows the output probability of identifying the real class of the target at different relative positions and a fixed relative orientation from the robot.
%         }} \label{fig:ObsModel}
% \end{figure}



% \begin{figure*}[t!] 
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/-180.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{-180 degrees}\label{fig:-180}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/-160.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{-160 degrees}\label{fig:-160}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/-140.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{-140 degrees}\label{fig:-140}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/-120.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{-120 degrees}\label{fig:-120}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/-100.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{-100 degrees}\label{fig:-100}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/-80.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{-80 degrees}\label{fig:-80}}
%         \end{subfigure}
%         % \hfill
%         ~

%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/80.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{80 degrees}\label{fig:80}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/100.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{100 degrees}\label{fig:100}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/120.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{120 degrees}\label{fig:120}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/140.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{140 degrees}\label{fig:140}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/160.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{160 degrees}\label{fig:160}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \captionsetup[subfigure]{position=b}
%         \begin{subfigure}{0.32\textwidth}
%                 \includegraphics[width=\textwidth]{sec/additional_content/obs_model/n2_class2/180.png}
%         %\vspace{-5mm}
%         \caption{\footnotesize{180 degrees}\label{fig:180}}
%         \end{subfigure}
%         % \hfill
%         ~
%         \caption{\footnotesize{Probability heat-map of the employed black-box classifier for a target of class 2. For a robot placed in the center, facing upwards, every plot shows the output probability of identifying the real class of the target at different relative positions and a fixed relative orientation.
%         }} \label{fig:ObsModel}
% \end{figure*}

==> sec/backup/backup_general.tex <==
%Although in this work each target has been assumed to belong to one class, it is easy to extend this formulation to the classification of each target into multiple classes requiring different sensor classifiers and observations from different perspectives. We leave the development of such formulation to future work.
% Also, in our formulation we have assumed each target to be independent of each other. The modelling and exploitation of target correlations in dynamic active classification will be left for future work.





==> sec/backup/backup_results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% backup images




\begin{figure*}[!t] % images on scenario progression (scenarios not training) (maybe reduce to 2 metrics, safety and communication) and final histograms. The other metrics can be used when evaluating the learned policy.
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/100_ts/ntracked_static.png}
        \caption{Static target dynamics.\label{fig:static}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/100_ts/ntracked_ctevel.png}
        \caption{Constant velocity target dynamics.\label{fig:ctevel}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/100_ts/ntracked_sfgoal.png}
        \caption{Social forces target dynamics.\label{fig:sfgoal}}
        \end{subfigure}
        % \hfill
        \caption{Comparison of our policy with the baselines in environments containing up to 55 targets. Our method has been trained as explained in section \ref{sec:method}. Our method scales better than the baselines with the number of targets, especially in environments where the targets' dynamics differ from the training conditions.} \label{fig:100tsenv}
        
\end{figure*}
\begin{figure*}[!t] % images on scenario progression (scenarios not training) (maybe reduce to 2 metrics, safety and communication) and final histograms. The other metrics can be used when evaluating the learned policy.
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/200_ts/ntracked_static.png}
        \caption{Static target dynamics.\label{fig:static200}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/200_ts/ntracked_ctevel.png}
        \caption{Constant velocity target dynamics.\label{fig:ctevel200}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/200_ts/ntracked_sfgoal.png}
        \caption{Social forces target dynamics.\label{fig:sfgoal200}}
        \end{subfigure}
        % \hfill
        \caption{Comparison of our policy with the baselines in environments containing up to 55 targets when doubling the amount of timesteps before timeout. Our method has been trained as explained in section \ref{sec:method}. These results prove that our method still outperforms the baselines even when more time is given to all methods to accomplish the task.} \label{fig:200tsenv}
        
\end{figure*}
In this section we describe our implementation of the proposed method and evaluate it in simulation.  %A







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t] % images on scenario progression (scenarios not training) (maybe reduce to 2 metrics, safety and communication) and final histograms. The other metrics can be used when evaluating the learned policy.
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/ntracked_static.png}
        \caption{Static target dynamics.\label{fig:static200}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/ntracked_cte_vel.png}
        \caption{Constant velocity target dynamics.\label{fig:ctevel200}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/ntracked_sf_goal.png}
        \caption{Social forces target dynamics.\label{fig:sfgoal200}}
        \end{subfigure}
        % \hfill

        
        \caption{Comparison of our policy with the baselines in environments containing up to 50 target.} \label{fig:firstperformance}
\end{figure*}

\begin{figure*}[!t] 
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/unclass_histogram_static.png}
        \caption{Static target dynamics (16 targets).\label{fig:static200}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/unclass_histogram_cte_vel.png}
        \caption{Constant velocity target dynamics (16 targets).\label{fig:ctevel200}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/unclass_histogram_sf_goal.png}
        \caption{Social forces target dynamics (16 targets).\label{fig:sfgoal200}}
        \end{subfigure}
        % \hfill
        
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/class_percentage_static.png}
        \caption{Static target dynamics (16 targets).\label{fig:static200}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/class_percentage_cte_vel.png}
        \caption{Constant velocity target dynamics (16 targets).\label{fig:ctevel200}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.33\textwidth}
                \includegraphics[width=\textwidth]{images/performance_scale/class_percentage_sf_goal.png}
        \caption{Social forces target dynamics (16 targets).\label{fig:sfgoal200}}
        \end{subfigure}
        % \hfill
        
        \caption{Comparison of our policy with the baselines along an episode in environments of 16 targets. a)-c) Plots the number unclassified targets simultaneously observed at each time step for each environment dynamics. The monotonically decreasing plots in d)-f) represents the percentage of classified targets along the episode for each method.} \label{fig:singleEpisodeperformance}
\end{figure*}



%Our method has been trained as explained in section \ref{sec:method}. These results prove that our method still outperforms the baselines even when more time is given to all methods to accomplish the task.

\section{Results}
In this section we describe the implementation and training of the proposed method. Next, we provide a thorough evaluation of the trained policy and analyze its robustness and scalability properties in comparison with other baselines.

\subsection{Training Setup and simulation environment} \label{results:trainingsetup_and_env}
We train our active classification motion planning policy for a robot moving in an $\mathbbm{R}^2$ environment of $16\times16 m^2$. During training, targets behave as particles with constant velocity dynamics, colliding elastically among themselves and against the limits of the environment. Targets are modelled as cylinders of $0.6m$ radius, $1.8m$ of height, and their maximum velocity is $1m/s$ in each direction of movement.  The simulation time step is set to have a length of $\Delta t = 0.25s$. The range of movement of the robot between timesteps depends respectively on its maximum velocity which we set to $v^{max} = 2~m/s$, and maximum angular velocity that we consider to be $\dot{\psi}^{max}=60^o/s$. Thus, we assume $\Delta p^{max} = v^{max}\Delta t=0.5~m$, and $\Delta\psi^{max} = \dot{\psi}^{max}\Delta t=15^o$.

We set the upper bounds for the robot's action to $\Delta p^{max} = 2$ and $\Delta\psi^{max} = 60^o$. The quadrotor is given a timeout of $T=100$ time steps to complete the task.

%Target $j$'s characteristic is modeled to be observable from its front view, which is determined by its direction of movement. 
In order to speed up the training and evaluation, considering that the perception module is not a contribution of the paper we have opted for using a simulated model of the black-box.
We have considered a synthetic pinhole camera with focal length equal to 400 pixels that acquires images of $640\times 480$ pixels.
For each target we consider only the half part of the cylinder that is facing forward and project it into the image frame, if it is visible from the camera perspective.
This generates an image of a trapezoid with area and skew depending on the relative position and orientation of the target.
We use these two parameters to determine the probability distribution of the observation over the class set, decreasing the probability of the true class exponentially with the skew and increasing it linearly with the area.
We also penalize heavily trapezoids that do not fit in the image.
%In section \ref{results:simulated observation model}, we further detail how we simulate the robot's field of view, target observation, occlusions and sensor $h$'s classification estimates.

The learning algorithm and the training of our policy are implemented in Tensorflow \cite{tensorflow}, using the RLlib framework \cite{liang2018rllib}. The policy and value function models follow the architecture detailed in section \ref{sec:policy_network} and were trained for $2.4e7$ steps in environments containing up to twelve targets, sampled uniformly (first phase). Then, they were further trained for $2e7$ steps in environments containing a random number between one to six targets (second phase). Both parts of the training were done using an Intel i9-9900 CPU@3.10GHz computer. The hyperparameters used for training are explained in Table~\ref{table:hyperparam}. Computing the policy actions takes less than $4ms$ per time step, which allows for a real-time implementation of the framework with a control frequency that can exceed 20Hz by far if necessary. Values for the reward weights were $w_{AC}=100$, $w_{class}=5$, $w_{ent}=1$, $w_{time}=0.3$, $w_{m}=0.01$. We consider a target to be classified once the belief over one of the classes surpasses the threshold $\tau=0.95$. We consider task success reward is received once during the episode. Episodes are finished after reaching the timeout $T$ time step or after successfully classifying all targets.

%for $2.4e7$ step
%for other $2e7$ steps

%we consider boolean variables, $l^j_t$ to describe targets that have already been classified within an arbitrary quality threshold, $\tau

%We train and test our method in environments where targets have only one characteristic to be classified ($H=1$)  with two possible classes ($\cC_{h_1}=2$). Target $j$'s characteristic is modeled to be observable from its front view, which is determined by its direction of movement. In section \ref{results:simulated observation model}, we further detail how we simulate target observation, occlusions and sensor $h_1$'s classification estimates. % THIS NEEDS TO BE CHANGED, NO LONGER NECESSARY AFTER EDUARDO'S CHANGES (H = 1 from the start and can be extended)

%Weights of the reward function


%The targets maximum speed is set to $v_^{target}_{max} = 1m/s$ in every direction while the robot's is set at $2m/s$ in every direction.


%\subsection{Simulated Observation Model}\label{results:simulated observation model} % EDUARDO




% The probability of the rest of the classes is uniformly distributed to guarantee that they sum up to 1.
% \begin{equation}
%     p_{b^*}^{j}=\dfrac{1}{C} + \gamma_1 0.5 \exp\left(-\dfrac{s}{20}\right) \min\left(\dfrac{a}{a_{\min}}, 1\right)
% \end{equation},
% where $\gamma_1$ is a correction factor of $0.1$ in case part of the trapezoid lies outside of the image.
% In summary, the probability is close to one for targets observed frontally, not too close and not too far away and approaches to.

\subsection{Performance evaluation}
% Explain in simulation environment the different target dynamics at test time.
We evaluate the performance of our method in environments presenting different amount of targets and different target dynamics: static, constant velocity and social forces dynamics. Social forces pedestrian dynamics are modeled after \cite{socialforces}. The idea of the latter is to test the robustness of our method to environments where the targets follow a different dynamic model than the one used in training.


Each policy is given a timeout of $T=200$ time steps and is evaluated by the percentage of targets it has been able to classify before the end of the episode. We define a set of baselines that we compare with our method: %The ablations are either modified versions of the baseline or our method:

\begin{itemize}    
    \item Hand-crafted: it is a hard coded policy that assumes a rough knowledge of where to observe a target from to find the information we want to classify. It classifies each target one-by-one by guiding the robot towards a pose that is 2m in front of the target, pointing the camera at it. Targets are prioritised by whether they have been already classified or not, then by proximity. Once a target has been selected the robot must classify it before choosing another one. Observations of targets other than the chosen one are still accounted for.
    \item Learned Single-Target: it is similar to the other baseline, only this one does not assume any knowledge on where informative viewpoints are placed with respect to the target. Thus, this policy learns from where to observe a target to classify the target as quickly as possible. For such task, the use of a 2-layer Multi-Layer Perceptron is more than enough. This baseline has been trained to convergence in scenarios with just one target following constant velocity dynamics. When confronted with multiple targets, it classifies each individually, following the same priority schedule as the previous baseline. Any observation of non-chosen targets are still accounted for to improve their respective beliefs.
    %\item Learned baseline v2 (ablation):
    %\item LSTM encoder (ablation):
    %\item DeepSets decoder (ablation):
\end{itemize}

We evaluate all the methods for 50 episodes in environments with 1 to 50 targets, for each one of the explained target dynamics, to evaluate them in both in-training and out-of-training scenarios. For the sake of fairness, we randomly sample the initial configuration for each combination of target quantity and dynamics, save it, and evaluate each policy under the same random initial conditions. For each plot, we have trained each learned policy with three different seeds and evaluated them. The shown results are the mean and standard deviations of the average results obtained for all three of them across all episodes.


In fig. \ref{fig:firstperformance} we report the percentage of targets that each method has been able to classify in every setting. In general, as expected, there is a drop in the percentage of targets that can be classified when their quantity and density increases. This is due to the fact that the task takes theoretically longer to complete and the number of occlusions among targets increases. This becomes even more apparent in static environments, where targets might be completely occluded by other targets or directly facing into a wall, making it more difficult, or even impossible, to classify them.

While our method behaves similarly to the learned baseline when targets are static, it clearly outperforms both baselines in dynamic environments. It not only performs well in scenarios seen during training, but it also manages to scale well and better to scenarios where the number and density of targets to classify is much greater than seen during training ($>$12 targets). When further monitoring the number of unclassified targets along the episode in scenarios with 16 targets (fig. \ref{fig:singleEpisodeperformance} a)-c)), during the first half of the episode, our method consistently is shown to observe and provide classification estimates of more targets than the baselines at every time step. Then, as targets get classified along the episode, the pool of unclassified ones grows smaller (as seen in d)-f)) and their viewpoints become sparsely distributed across the environment. This is the reason why the number of unclassified targets that can be observed simultaneously with minimal time step and movement cost drops significantly.

Our architecture is able to account for all targets' available information at the same time. This means that it is able to learn strategies that prioritise to go towards viewpoints allowing simultaneous observations of multiple unclassified targets, even if that means losing classification accuracy for some of them. Additionally, the baselines are bound to classify the targets following a heuristic proximity-based priority order. This order of priority might not be the best one, as it should depend on the relative pose and velocity of the targets with respect to the camera and the classifier sensor model. However, we do not have access to the latter and both baselines cannot reason about all targets' information at the same time, which is why these results show that, at least, our method is able to learn a better classification priority order.

It is also remarkable to see that the method is able to generalize and perform well when the targets follow other dynamics than seen during training. This is probably due to the fact that targets under social forces behave similarly to their constant velocity counterpart when traveling to their goals. Also, due to the repulsive force of dynamic and static obstacles (targets and walls), it is not likely for two targets to be facing each other or against a wall. This makes it easier for our method to find suboptimal viewpoints allowing to obtain good classification estimates of multiple targets at a time. In contrast, the learned baseline is not robust to this change in dynamics as it cannot learn to avoid target occlusions.

In fig. \ref{fig:horizonanalysis}, we provide results on the baselines and our method's performance under different timeout conditions in scenarios with 16 targets with constant velocity dynamics. It shows empirical proof that our method is able to complete the task if given enough time. Also, we show that our proposed method is able to approach the end of the task generally faster than the baselines. 

\begin{figure}[t!]
    \centering
    \includegraphics[width=8.5cm]{images/horizon/horizon_analysiscte_vel.png}
    \caption{Performance of for 16 targets following constant velocity dynamics when the length of an episode (timeout) is varied. Note that all methods learn to classify all targets eventually, but that our approach is much faster.
    %Timeout analysis in scenarios of 16 targets following constant velocity dynamics.
    }
    \label{fig:horizonanalysis}
\end{figure}

\subsection{Ablations}
Next we compare the performance of our method with that of ablated architectures. While there are architectures in the learning-based motion planning literature that map environment representations of an arbitrary dimension to a latent representation vector of fixed dimension, these methods are either not permutation invariant \cite{britogompc}, or weight each element in the input sequence equally \cite{Hsu2021}. We argue that these are important biases that must be encoded into our architecture for it to be more robust and consistent. Inspired by these two works, we design ablated versions of our architecture that mirror the architectural choices in these two works and train them following the same training schedule we use for our method :
\begin{itemize}    
    \item LSTM encoder (ablation): every element is inversely sorted by proximity to the robot and depending on whether they have been classified (already classified targets that are far away go first). Then every element in the sequence is mapped to its latent representation using a linear encoder. Then the whole sequence is fed to an LSTM layer so that the nearest target's latent representation is fed the last. This ensures that the memory vector in the LSTM retains more information about the closest (and assumed to be more relevant) target and less about the furthest. This policy assumes and enforces an order in the input sequence. While in safe navigation tasks proximity is a good estimate to determine priority, this is cannot be trivially assumed in active classification tasks.
    \item DeepSets decoder (ablation): We replace the $PMA_1$ layer of our architecture by a mean pooling layer. Following \cite{NIPS2017_f22e4747} and similar to the architecture described in \cite{Hsu2021}, it is equivalent to having an self-attention block as an encoder function, and a multi-layer perceptron as a decoder. In contrast to the previous ablation, this method does not assume any kind of priority in the attention every target's latent representation receives. This is not accurate, specially in active classification where, for starters, there is a set of targets that have already been classified and targets that still remain to be classified, and therefore their observation should be prioritized.
\end{itemize}

In Fig. \ref{fig:ablations}, we show how these ablations scale and generalize to scenarios not seen during training, having an increasing amount of targets following social forces dynamics. While both ablations show good performance, our method, thus architecture choice, outperforms both of them, showing better scalability properties in scenarios that none of the policies have seen before.


\begin{figure}[t!] % MUST BE UPDATED
    \centering
    \includegraphics[width=8.5cm]{images/ablations/ntracked.png}
    \caption{Comparison of our method with ablations.}
    \label{fig:ablations}
\end{figure}


==> sec/backup/biblio.tex <==
@inproceedings{
andrychowicz2021what,
title={What Matters for On-Policy Deep Actor-Critic Methods? A Large-Scale Study},
author={Marcin Andrychowicz and Anton Raichuk and Piotr Sta{\'n}czyk and Manu Orsini and Sertan Girgin and Rapha{\"e}l Marinier and Leonard Hussenot and Matthieu Geist and Olivier Pietquin and Marcin Michalski and Sylvain Gelly and Olivier Bachem},
booktitle={International Conference on Learning Representations},
year={2021},
}

@INPROCEEDINGS{efficientMultiview,
  author={Xu, Qianli and Fang, Fen and Gauthier, Nicolas and Liang, Wenyu and Wu, Yan and Li, Liyuan and Lim, Joo-Hwee},
  booktitle={IEEE Int. Conf. on Robotics and Automation}, 
  title={Towards Efficient Multiview Object Detection with Adaptive Action Prediction}, 
  year={2021},
  pages={13423-13429},
  doi={10.1109/ICRA48506.2021.9561388}}
  
  @inproceedings{NIPS2017_3f5ee243,
 author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
 booktitle = {Adv. in Neur. Inform. Processing Systems},
 pages = {1-11},
 title = {Attention is All you Need},
 volume = {30},
 year = {2017}
}

@InProceedings{10.1007/978-3-319-93417-4_38,
author={Schlichtkrull, Michael
and Kipf, Thomas N.
and Bloem, Peter
and van den Berg, Rianne
and Titov, Ivan
and Welling, Max",
editor="Gangemi, Aldo
and Navigli, Roberto
and Vidal, Maria-Esther
and Hitzler, Pascal
and Troncy, Rapha{\"e}l
and Hollink, Laura
and Tordai, Anna
and Alam, Mehwish},
title="Modeling Relational Data with Graph Convolutional Networks",
booktitle="The Semantic Web",
year="2018",
publisher="Springer International Publishing",
address="Cham",
pages="593--607",
isbn="978-3-319-93417-4"
}

@inproceedings{liang2018rllib,
    Author = {Eric Liang and
              Richard Liaw and
              Robert Nishihara and
              Philipp Moritz and
              Roy Fox and
              Ken Goldberg and
              Joseph E. Gonzalez and
              Michael I. Jordan and
              Ion Stoica},
    Title = {{RLlib}: Abstractions for Distributed Reinforcement Learning},
    Booktitle = {Int. Conf. on Mach. Lear.},
    Year = {2018}
}

@inproceedings{
Engstrom2020Implementation,
title={Implementation Matters in Deep RL: A Case Study on PPO and TRPO},
author={Logan Engstrom and Andrew Ilyas and Shibani Santurkar and Dimitris Tsipras and Firdaus Janoos and Larry Rudolph and Aleksander Madry},
booktitle={Int. Conference on Learning Representations},
year={2020},
}


==> sec/backup/implementation_backup.tex <==
\section{Implementation}

\subsection{Training environment and algorithm}

In dynamic active classification problems, we identify two possible situations that require different behaviors. The first one is generally experience in environments with low target quantity (1 to 6 targets), where simultaneous observations are difficult to obtain. Therefore, the robot will have navigate to locations where one target can be observed at a time. The second one applies to situations where multiple unclassified targets can be identified simultaneously, which generally happens in scenarios with a higher number of targets ($>$6 targets). In this case, the robot will benefit from moving to viewpoints that avoid occlusions and allow simultaneous observations, rather than moving to single target viewpoints. For this reason, we follow a two-phase training schedule. First, we train the policy for the general case in scenarios, chosen randomly, containing from 1 to 12 targets. Then we further refine the resulting policy by training it in scenarios containing from 1 to 6 targets.

%There are mainly two possible active classification strategies. The first one applies generally to low target quantity (1 to 6 targets) scenarios, where informative viewpoints are sparse. Therefore, the robot will have to observe one target and/or characteristic at a time. The second one applies to situations where multiple unclassified targets can be identified simultaneously, which generally happens in scenarios with a higher number of targets ($>$6 targets). In this case, the robot will benefit from simultaneous observations rather than moving to single target viewpoints. For this reason, we follow a two-phase training schedule. First, we train the policy in scenarios, chosen randomly, containing from 1 to 12 targets. Then we further refine the resulting policy by training it in scenarios containing from 1 to 6 targets. 

%for $2.4e7$ step
%for other $2e7$ steps
% Dos casuisticas identificables  de estrategias.

During training, targets follow constant velocity with orientation equal to the orientation of motion, having elastic collisions whenever they collide against walls or other targets. We assume the quadrotor can go faster than the targets. This is to ensure that the quadrotor can reach targets that are going away from him. Following the ideas of \cite{domainRandomization}, we randomize the robot and targets' initial poses, the targets' initial velocities and the beliefs over their classes, which means that some targets might randomly be classified from the start. Some of the targets are randomly selected and enforced to remain static. This is to enhance state space exploration, which will make the learned policy more robust at test time.

%The targets maximum speed is set to $v_^{target}_{max} = 1m/s$ in every direction while the robot's is set at $2m/s$ in every direction.


For training our policy, we use the on-policy policy gradient algorithm Proximal Policy Optimization (PPO)~\cite{schulmanPPO}. The algorithm alternates between gathering experiences $(\vo_t,\va_t,R(\vs_t,\va_t),\vo_{t+1})$ and performing PPO gradient updates. PPO is an on-policy method that addresses the high-variance and the difficult hyperparameter tuning in policy gradient methods for continuous control problems. We use the PPO implementation from the RLlib framework \cite{liang2018rllib} that combines both a clipped surrogate loss and a Kullback–Leibler divergence term to make sure the updated policy is not too different in terms of action probability distribution. As suggested in \cite{schulmanPPO}, we add to the surrogate objective an entropy regularization term and a value function loss to ensure sufficient exploration. We refer the reader to \cite{schulmanPPO} for more information on the method's equations and details. The hyperparameters used for training are shown in table \ref{table:hyperparam}.

\begin{table}[t]
    \centering
    \caption{Hyperparameters for PPO training algorithm}
    \begin{tabular}{|c|c|}
    \hline
        Parameter & Value \\
    \hline
        Lambda $\lambda$ & 0.95 \\
        Gamma $\gamma$ & 0.99 \\
        Time steps each update & 4000 \\
        %Episode time steps/episode $T_e$ & 100 \\
        Number of epoch per update & 30 \\
        SGD minibatch size & 256 \\
        PPO Clip param. & 0.3 \\
        KL target & 0.01 \\
        Learning rate & 3e-4 \\
        KL coeff. & 0.2 \\
        Value function loss coeff. & 1 \\
        Entropy loss coeff. $c_2$ & 0.001 \\
        Gradient Clipping & 0.1 \\
    \hline
    \end{tabular}
    \label{table:hyperparam}
\end{table}

% - Dynamics
% - Domain randomization
%   - initial positions, velocities, beliefs and number of targets
% - No access to the observation model
% - Training done in two phases: 1st trained for 2.4e7 ts, 2nd trained for 2e7 ts




\subsection{Training Setup and simulation environment} \label{results:trainingsetup_and_env}
We train our active classification motion planning policy for a robot moving in an $\mathbbm{R}^2$ environment of $16\times16 m^2$. During training, targets behave as particles with constant velocity dynamics, colliding elastically among themselves and against the limits of the environment. Targets are modelled as cylinders of $0.6m$ radius, $1.8m$ of height, and their maximum velocity is $1m/s$ in each direction of movement.  The simulation time step is set to have a length of $\Delta t = 0.25s$. The range of movement of the robot between timesteps depends respectively on its maximum velocity which we set to $v^{max} = 2~m/s$, and maximum angular velocity that we consider to be $\dot{\psi}^{max}=60^o/s$. Thus, we assume $\Delta p^{max} = v^{max}\Delta t=0.5~m$, and $\Delta\psi^{max} = \dot{\psi}^{max}\Delta t=15^o$.

We set the upper bounds for the robot's action to $\Delta p^{max} = 2$ and $\Delta\psi^{max} = 60^o$. The quadrotor is given a timeout of $T=100$ time steps to complete the task.

%Target $j$'s characteristic is modeled to be observable from its front view, which is determined by its direction of movement. 
In order to speed up the training and evaluation, considering that the perception module is not a contribution of the paper we have opted for using a simulated model of the black-box.
We have considered a synthetic pinhole camera with focal length equal to 400 pixels that acquires images of $640\times 480$ pixels.
For each target we consider only the half part of the cylinder that is facing forward and project it into the image frame, if it is visible from the camera perspective.
This generates an image of a trapezoid with area and skew depending on the relative position and orientation of the target.
We use these two parameters to determine the probability distribution of the observation over the class set, decreasing the probability of the true class exponentially with the skew and increasing it linearly with the area.
We also penalize heavily trapezoids that do not fit in the image.
%In section \ref{results:simulated observation model}, we further detail how we simulate the robot's field of view, target observation, occlusions and sensor $h$'s classification estimates.

The learning algorithm and the training of our policy are implemented in Tensorflow \cite{tensorflow}, using the RLlib framework \cite{liang2018rllib}. The policy and value function models follow the architecture detailed in section \ref{sec:policy_network} and were trained for $2.4e7$ steps in environments containing up to twelve targets, sampled uniformly (first phase). Then, they were further trained for $2e7$ steps in environments containing a random number between one to six targets (second phase). Both parts of the training were done using an Intel i9-9900 CPU@3.10GHz computer. The hyperparameters used for training are explained in Table~\ref{table:hyperparam}. Computing the policy actions takes less than $4ms$ per time step, which allows for a real-time implementation of the framework with a control frequency that can exceed 20Hz by far if necessary. Values for the reward weights were $w_{AC}=100$, $w_{class}=5$, $w_{ent}=1$, $w_{time}=0.3$, $w_{m}=0.01$. We consider a target to be classified once the belief over one of the classes surpasses the threshold $\tau=0.95$. We consider task success reward is received once during the episode. Episodes are finished after reaching the timeout $T$ time step or after successfully classifying all targets.




==> sec/backup/intro_backup.tex <==

Multi-target tracking is a relevant problem in surveillance, patrolling and pursuit with mobile robots (citations), where a team of robots are tasked with searching and tracking several targets, such as other robots or humans. Having a good estimate of the target's state allows to react and plan for better strategies in the former and safe navigation tasks. However, to the best of our knowledge, these works tend to consider that all targets need to be tracked with the same priority and show little interest in the additional semantic information that can be extracted from observing the targets. \\

Tracking semantic target information may enable to solve more general problems. For example, knowing specific information about the targets in persistent monitoring applications may allow us to know if a target should be tracked and with what priority should we track it. Furthermore, recent works in computer vision using Deep Learning (DL) open the door to very interesting applications in the robot perception field. Specially, DL applications on image detection and semantic understanding may one day be used as general sensors that can identify and detect multiple characteristics from our targets. Nevertheless, these models are hard to characterize. In particular, it is generally difficult to model how the accuracy of these sensors changes or even if we can obtain the information of interest given a the relative position and orientation from our robot to the targets.\\

In this work, we aim to solve the perception and motion planning challenges described previously. Given a mobile robot, a set of multiple targets and their associated set of semantic information (e.g. eye color, hair length, ...) and a set of black box sensors (e.g. neural network-based detectors), we aim to develop a motion planning framework that:
\begin{enumerate}
    \item guides a mobile robot towards informative target viewpoints where correct detections with high confidence are obtained with high probability.
    \item maintains a belief over this information that is robust to wrong detections even when they are obtained with high confidence.
    \item is able to adapt to increasing number of targets.
\end{enumerate}

Our main challenge is the lack of a sensor model to exploit and compute optimal informative viewpoints over targets and the dependence of our detections on the relative pose between our robot and the targets. Therefore, we intend to  learn a policy that, given the current state and a set of beliefs over a set of targets' semantic information, guides our robot towards locations that provide useful observations of the target, lowering the uncertainty over the beliefs.


%can yield high confidence correct detections with high probability to lower the uncertainty over the beliefs





==> sec/backup/problem_form_backup.tex <==
\section{Preliminaries}
\subsection{Problem formulation} \label{sec:prelim_problemformulation}
%The ideal problem that we would like to solve involves solving the problem of gathering information with semantic meaning over  multiple targets with multiple robots. We formulate the following problem.\\

Consider a quadrotor $i$ with a camera that allows it to capture visual information inside an arc of radius $r_{obs}$ and angle $\theta_{obs}$ in front of it. The camera is assumed to be stabilised and can rotate independently from the robot. Let $\mathcal{J} = \{1,2,...,M\}$ be a set of dynamic targets and $\cH = \{h_1,h_2,...,h_H\}$ the set of sensor functions available to the robot, each able to capture and classify specific information target observations into $C_h, h\in\cH$ different categories. The state of the robot and targets are respectively represented by the sets $\vx$ and $\vy = \{\vy^1,\vy^2,...,\vy^M\}$, where states $\vx = [\vp^i, \vv^i, \psi^i]$ and $\vy^j = [\vp^j, \vv^j, \psi^j]$ are represented by the positions $\vp$, velocities $\vv$ and headings $\psi$ of each element. For the mobile robot, $\psi$ represents the heading of the camera. The quadrotor is assumed to fly above the targets. Therefore, we assume that targets may collide among themselves but not against the robot. Also, other targets can occlude the observation over targets behind them (from the camera's perspective). %The field of view of each robot depends on its state and is defined by the set $\mathcal{O}(\vx^i)$. Whether a target $j$ is inside the field of view of robot $i$ is modeled through an indicator function $\mathbbm{1}_{\mathcal{O}(\vx^i)}(\vy^j)$. The joint visibility of robot $i$ over all targets is represented by the set $\vz^i = \{\vz^{j|i}|\vz^{j|i}=\mathbbm{1}_{\mathcal{O}(\vx^i)}(\vy^j),\hspace{0.05cm}j\in\mathcal{J}\}$.\\ 

 %$\cH = \{1,2,...,H\}$ 

We assume no global positioning of the robot. Every time-step robot $i$ has available information of its own position and heading, observing the environment through its local reference frame, which moves and rotates with the camera.  We also assume it has available information on the relative states $\tilde{\vy}^j = [\tilde{\vp}^{j}, \tilde{\vv}^{j}, \tilde{\psi}^{j}]$ (relative position, velocity and orientation) of each target $j$. The joint relative state of all targets is defined by $\tilde{\vy} = \{\tilde{\vy}^j | j\in\cJ \}$

Each dynamic target has a set of characteristics $\vb^j = \{b_{1}^j,b_{2}^j,...,b_{H}^j\}$ (e.g. eye colour), where each element $b_{h}^j$ can take any value over the set of categories $\cC_h = \{1,...,C_h\}$ that sensor $h$ has been trained to classify (e.g. brown, blue, green). Every sensor is assumed to able to produce both a probabilistic classification estimate and the uncertainty of such estimate. Every time step, every sensor $h$ provides a probability distribution of target $j$ belonging to each class $c_h\in\cC_h$:
\begin{equation} \label{probability_estimate}
\mathbbm{P}(b_{h}^j = c_h) = 
     \begin{cases}
       h(c_h,\tilde{\vy}^j) & j~observable\\
       \frac{1}{C_h} & otherwise\\
     \end{cases}
\end{equation}
Where sensor $h$ outputs a probability distribution resulting from leveraging classification estimates with the uncertainty of such measurements. Such uncertainty depends on how much relevant information and the quality of observations we can get from target $j$. Note that being observable does not only depend on being inside the field of view, but also on not being occluded by other targets. However, since sensor $h$ is assumed to be a black-box classifier, we do not have access to $h$'s model and cannot state any dependency on $h$ other than target $j$'s visibility and relative pose. Note that information on each characteristic is generally not observable from all angles nor are always observable from the same perspective. The joint set of class probability distributions estimated at time step $t$ for every target $j$ and sensor $h$ is defined as $\vect{P}_t = \{\vect{P}_{h,t}^j | \forall j\in\cJ,~h\in\cH\}$ with $\vect{P}_{h,t}^j = \{\mathbbm{P}(b_{h}^j = c_h) | \forall c_h\in\cC_h\}$.

Sequential sensor class estimates for target $j$, $\vect{P}_t^j = \{\vect{P}_{h,t}^j | \forall h\in\cH\}$  are fused to build a set of target class beliefs $\tilde{\vb}^j = \{\tilde{\vb}_{1}^j,\tilde{\vb}_{2}^j,...,\tilde{\vb}_{H}^j\}$, each of which is associated to each target $j$'s characteristics. Each $\tilde{\vb}_{h}^j$ represents a probability distribution over the different categories that target $j$ can be classified into under sensor $h$. We define the joint set of beliefs over targets $\tilde{\vb}$. In summary, the available information for robot $i$ at time step $t$ is represented by the vector $\vo_t = [\tilde{\vy}_t, \vect{P}_t, \tilde{\vb}_t]$

In this work, we formulate the dynamic multi-target active classification task with uncharacterized sensors as a sequential decision-making problem that the robot solves at every timestep $t$. We take an information gathering perspective, with the objective being to maximize the mutual information between the history of robot sensor class estimates $\vect{P}_t$ and the targets' class information $\vb$. More formally, the goal of this work is to learn a mapping $\mathcal{F}$ that takes robot $i$'s available information ($\vo_t$), and determines an appropriate action ($\va_t$). We want the action $\va_t = \mathcal{F}(\vo_t)$ to be such that it contributes to the global objective of moving the robots towards viewpoints that will allow to maximise the future cumulative mutual information between the targets' class information and the history of the robot's class estimates given a time limit $T$, while accounting for target dynamics and occlusions. As described in equation \ref{problemformulation}:

\begin{equation} \label{problemformulation}
\begin{split}
    & \max_{a_{0:T-1}}\sum_{t=1}^{T}I(\vb;\vect{P}_{1:t}|\vx_{1:t})\\
    \text{s.t.} &\\
    & \vx_{t+1}=f(\vx_t,\va_t), \hspace{0.75cm} t=0,...,T-1\\
    & \vy^j_{t+1}=g(\vy^j_t), \hspace{1.30cm} t=0,...,T-1,~\forall j\in\cJ\\
    %& \vz^i_{t}=\mathbbm{1}_{\mathcal{O}(\vx^i_t)}(\vy_t), \hspace{2.65cm} t=1,...,T
    %& \tilde{\vb}^i_{t+1}=q(\tilde{\vb}^i_{t},\vz^i_{t}|\vb^i_{t},\vx^i_t,\vy_t), \hspace{0.85cm} t=0,...,\infty\\%T
    %& OR \\
    & \tilde{\vb}_{t}=q(\tilde{\vb}_{t-1},\vect{P}_{t}), \hspace{0.75cm} t=1,...,T\\
\end{split}
\end{equation}
where $f$ is the dynamics of our mobile robot, $g$ is the dynamics of our targets, and $q$ is the function that models how the beliefs are updated given the current sensor class estimations. Beliefs are initialized at $t=0$ with an uniform prior over categories.

We assume characteristic from target $j$ has been classified if, at time t, there exists any $c_h$ for which $\tilde{\vb}_{h,t}^j(b_{h}^j = c_h) \geq 0.95$. We denote this condition by the boolean variable $l^j_{h,t}$. The set of boolean variables for target $j$ is denoted by $\vl^j_t = \{l^j_{h,t} | \forall h\in\cH\}$.

%\mathbbm{1}\{\tilde{\vb}_{h}^j(b_{h}^j = c_h) \geq 0.95\}(\tilde{\vb}_{h}^j)$\\

%This problem is too complex to address directly. Our aim is to first solve this problem for one agent and multiple targets in an environment without obstacles. Occlusions in the robot's observations only happen due to another target being in the way. Alternatively, if we're in need of a simpler setting, we can consider the drone to operate above the targets, which may avoid inter-target occlusion.

% and the robots' future observations,

%is modeled as a one-hot vector and represents the category of target $j$'s information that sensor/detector $s\in\cS$ has been trained to identify. The dimensionality of the one-hot vector depends on the number of categories $\cC_s = \{1,...,C_s\}$ that sensor $s$ can classify

%where each element 

%over the set of possible categories that sensor s can identify

%on whether the robot can observe the target and the relative orientation of the target with respect to the camera

%under which instances of this piece of information can be classified

%Every time a sensor makes a detection, we assume without loss of generality that it  Such classifications\\ %\cite{}.\\


%% part on classifications of sensor s


%A framework for multi-view active classification extended to dynamic targets, that can be combined with the use of uncharacterized sensors (e.g. black-box classifiers) as long as classification uncertainty can be estimated.

%In this work, we formulate the dynamic multi-target semantic information gathering with uncharacterized sensors as a sequential decision-making problem that each robot solves at every timestep $t$, with the objective of maximizing the mutual information between the robots' observations $\vz_t$ and the targets' semantic information $\vb$. More formally, the goal of this work is to learn a mapping $\mathcal{F}$ that takes the available information from each robot ($\vo_t = \{\vo^1_t,...,\vo^n_t\}$), and determines an appropriate action for each of them ($\vu_t = \{\vu_t^1,...,\vu_t^n\}$). We want the action $\vu_t = \mathcal{F}(\vo_t)$ to be such that it contributes to the global objective of moving the robots towards positions that will allow them to maximise the future cumulative mutual information between the targets' semantic information and the robots' future observations, to the best of the teams capabilities. This is described in equation \ref{problemformulation}:

% This function has information that you don't have, if you don't know the uncertainty matrix we cannot use the kalman filter for planning.
% Make two descriptions of the problem that we're trying to solve

%\subsection{Conflation of probability distributions}\label{sec:prelim_conflation} %EDUARDO

\cite{Hill2011,Hill2008}

%%%%%%%%%%%%%%%%%%%%%%%
\section{Our approach and Requirements}
\begin{itemize}
    \item RL for subgoal recommendation and camera control, MPC for motion planning.
    \item Permutation invariant architecture capable of processing an arbitrary number of target's information.
    \item Keep and update beliefs using detections and confidence of detections as a reference to provide a direction and step-size for the update (Bayesian update not possible).
    \item Reward produced from tracking the belief entropy decrease produced by new detections, and the correctness of our beliefs.
\end{itemize}

% THIS GOES IN THE APPROACH SECTION%The objective is to learn a policy that performs as well as a coupled centralized expert, while restricting robots to their decentralized policies.\\

%They also have available information on the joint monitoring score from all targets $\mathbf{s}_G$. We define the available information for robot $i$ at timestep $t$ as $\mathbf{o}_i^t = (\mathbf{v}_i^t,\mathbf{p}_{-i}^t, \mathbf{v}_{-i}^t, \mathbf{p}_G^t,\mathbf{v}_G^t, \mathbf{s}_G^t)$. All robots can communicate with each other.

%%%% Wendeling Notes

- Things missing: in equation (1) I need to put the dynamics of the beliefs.
- Do not have the info to build a kalman filter, we can only build smth based on sampling the detector.
- Belief system -> threshold system to say whether we are certain or not about 
- Describe task in different abstraction levels
1. Identify n features in m targets, we want to know whether target j has feature s -> RL
2. Lower level ignore the part over the belief deciding where the robot should go. I assume that the -I want a belief on the real world that is as close as possible to the real world.
3. We need to define a task as a subset of semantic information of interest that we want to track.
4. We have smth in here that we dont know in practice. We assume that the belief we have over smth is justified. 


==> sec/backup/related_work_backup.tex <==
\section{Related Works and Contribution}

Our contributions build upon recent work in multi-view active classification and learning for motion planning in dynamic environments.

%\subsection{Multi-view active classification}

\subsection{Multi-view active classification}~~~~The problem of active classification is typically solved by pre-defining a set of viewpoints through which trajectories are planned to gather sufficient information to solve an active classification task. %\cite{activeWeedClassification,Natansov2014,Patten2016ViewpointEF,Patten2018,activePerceptionAutonomousObservation}. 
One-step greedy planners have been used for active object classification~\cite{Patten2016ViewpointEF}. Given a set of viewpoints for each object, these works select the most informative one based on a utility function that depends on the
%associate an utility to each viewpoint depending on the %estimated viewpoint utility (which depends on a predefined training set), 
object class uncertainty and the observation occlusion. %The viewpoint with maximum utility is selected. 
Non-myopic methods that account for the cost of movement between viewpoints have also been developed to solve the problem of active classification. For example,~\cite{activeWeedClassification} takes an Informative Path Planning approach, assuming a known classification uncertainty model, to plan trajectories over a pre-defined viewpoint lattice.
%that depends on the class and distance to the target. It uses a pre-defined viewpoint lattice to generate and refine trajectories that minimize the uncertainty over the target class. 
Alternatively,~\cite{Natansov2014} formulates the problem as a partially observable Markov Decision Process (POMDP) and plans a path over viewpoints while leveraging the cost of making a new measurement against the probability of making a wrong classification and accounting for occlusions. With a similar formulation,~\cite{Patten2018} proposes a variation of Monte Carlo tree search to plan non-myopically. %However, 
These methods generally assume access to an observation model that allows to estimate viewpoint usefulness a priori. In this work, we consider the case in which a black box classifier is employed and do not have access to this model. %since we intend to use a black box classification approach.

Learning methods allow to obtain non-myopic solutions for static targets while using black-box models. Recent works have leveraged the use of Deep Reinforcement Learning for multi-target pose estimation and active classification by learning a policy that guides the camera towards viewpoints %observing the object it is most uncertain about
that reduce observation uncertainty~\cite{active6D} or learning to move the camera to observe a set of targets from multiple viewpoints and enhance their classification accuracy~\cite{efficientMultiview}. Nevertheless, these methods assume that the targets to be classified are static, which makes them unsuitable for active classification with moving targets.

%\subsection{Dynamic target visibility}
To deal with dynamic targets,~\cite{activePerceptionAutonomousObservation} considers a pre-defined set of viewpoints distributed along a closed environment.% and formulate the autonomous observation problem as a Semi-Markov Decision Process to maximize an observation score over moving humans. However, it is restricted to a predefined closed environment. %to a limited working environment.
Works in the field of aerial videography are generally not bound by a closed environment~\cite{ALCANTARA2021103778, detectionAware}. Yet, such approaches tend to focus on target visibility instead of improving target classification. This would require to know in advance from which perspective each dynamic target needs to be observed, which might not be available or well-modeled.

%as they optimize for visibility under occlusion while ensuring collision-free trajectories together with cinematographic aspects~\cite{ALCANTARA2021103778}.
% Recent works in this field leverage the use of optimization methods in order to generate trajectories that allow common visibility of multiple targets~\cite{Nageli2017, Boseong2021} and provide multi-view shots over a scene~\cite{Bucker2021DoYS,NageliMeier}. 
%Most related to our approach,~\cite{detectionAware} employs a detectability objective which encourages the generated trajectories to include viewpoints where the target is well-distinguished against the colors of the background. Yet, such approaches tend to focus on target visibility instead of improving target classification. This would require to know in advance from which perspective each dynamic target needs to be observed, which might not be available or well-characterized.


%\subsection{Learning for motion planning in dynamic environments}

\subsection{Learning for motion planning in dynamic environments}~~~~Learning approaches in motion planning tasks have the potential to encode and identify patterns in the state space in complex motion planning tasks. Recent advances in Deep Representation Learning show promise in learning latent representations of the state space, capturing the underlying structure and symmetries in dynamic environments~\cite{GeometricDL}. Recent works in learning-based motion planning policies rely on Convolutional Neural Networks (CNN)~\cite{DenseCAvoid,cui2021} for visual-based navigation or encode the state of multiple and variable static/dynamic elements in the environment using Graph Convolutional Networks (GCN)~\cite{Li2019,Chenyuying}, Long-Short Term Memory layers (LSTMs)~\cite{britogompc,meverett2021,Chen2017SociallyAM} and self-attention based architectures~\cite{Chen2019}.% to encode and navigate through complex dynamic environments. 

%However, 
LSTMs assume an order in the sequence of elements encoded, which makes it hard to treat symmetries in the state space. Instead, GCN and DeepSets~\cite{NIPS2017_f22e4747} are permutation invariant function approximators since they process the information of each element sequence independently of the order they are arranged. Nevertheless, GCNs require accurate prior knowledge of the encoded graph structure~\cite{kurin2021my} while DeepSets assign equal weight to each element in the decision making process.

Most related to our approach,~\cite{Hsu2021} uses a combination of Self-attention~\cite{NIPS2017_3f5ee243} and DeepSets~\cite{NIPS2017_f22e4747} to learn a policy that learns to coordinate a multi-robot system to track a set of dynamic targets. Yet, DeepSets aggregates all targets' information by assigning equal weights to them. In contrast, we leverage the use of self-attention~\cite{NIPS2017_3f5ee243} and attention-based permutation-invariant set-function approximators~\cite{lee2019set} to effectively encode the dynamic environment, learning the importance of each target in our future decision.

%\subsection{Contribution}
%where informative observations are restricted to particular relative orientations between the robot and targets
%\textbf{Contribution}~~~~



% We formulate the active classification objective %of multi-view active classification of dynamic targets with black-box classifiers 
% as a sequential decision-making problem. We then solve it by employing Deep Reinforcement Learning to learn an attention-based control policy that performs the classification over an arbitrary number of dynamic targets. Observations of unclassified targets are combined sequentially until a robust estimate of their class is achieved. Since informative observations are restricted to a set of relative target orientations, the learned policy trades-off observations of unclassified targets with the informativeness of such observations. % The learned policy is able to scale up with the number and density of targets in the environment.

% We compare our method in a simulated environment against other hand-engineered and learned baselines and analyze its ability to scale to different amounts of targets than those seen during training. %Some of the presented baselines encode the environment using architectures that have been successfully applied in the collision avoidance task~\cite{britogompc,meverett2021,Hsu2021}.
% Furthermore, we evaluate the scalability and tracking performance of the proposed method against the baselines under different motion dynamics of the targets, which have not been seen during training, and we analyze the behavior of our learned policy. 

%uncharacterized sensors (e.g. black-box classifiers)



% \textbf{Contribution}~~~~We formulate the problem of active classification of dynamic targets with black-box sensors as a sequential decision making problem. We then solve the problem by employing Deep Reinforcement Learning to learn an attention-based control policy that is able to perform active classification on an arbitrary number of dynamic targets. Observations over unclassified targets are combined sequentially until a robust estimate of their class is achieved. Since informative observations are restricted to a set of relative target orientations, the learned policy trades-off observations of unclassified targets with the informativeness of such observations. % The learned policy is able to scale up with the number and density of targets in the environment.

% The main contributions of this work are:
% \begin{itemize}
%     \item A framework for multi-view active classification extended to dynamic targets, that can be combined with the use of black-box classifiers.% as long as classification uncertainty can be estimated.
%     \item A novel attention-based architecture that can learn to adapt to different target configurations and scale to scenarios presenting large target quantities and densities.
% \end{itemize}

% We compare our method in a simulated environment against other hand-engineered and learned baselines and analyze its ability to scale to different amounts of targets than seen during training. %Some of the presented baselines encode the environment using architectures that have been successfully applied in the collision avoidance task~\cite{britogompc,meverett2021,Hsu2021}.
% Furthermore, we evaluate the scalability and tracking performance of the proposed method against the baselines under different moving dynamics of the targets, some of which have not been seen during training, and we analyze the behavior of our learned policy. 



% To the best of our knowledge, we address for the first time the challenge of active classification with dynamic targets without having available an observation model.

==> sec/figure_realistic.tex <==
\begin{figure*}[b!] 
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.32\textwidth}
                \includegraphics[width=\textwidth]{images/corl/performance_airsim/ntracked_75s.png}
        \vspace{-5mm}
        \caption{\footnotesize{}\label{fig:scalabilityReal}}
        \end{subfigure}
        % % \hfill
        % ~
        % \captionsetup[subfigure]{position=b}
        % \begin{subfigure}{0.32\textwidth}
        %         \includegraphics[width=\textwidth]{images/corl/performance_airsim/class_percentage_airsim_realistic.png}
        % \vspace{-5mm}
        % \caption{\footnotesize{}\label{fig:MissclassReal}}
        % \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.32\textwidth}
                \includegraphics[width=\textwidth]{images/corl/performance_airsim/class_percentage_airsim_photoreal_simu_teleport.png}
        \vspace{-5mm}
        \caption{\footnotesize{}\label{fig:classificationspeedRealPerception}}
        \end{subfigure}
        % \hfill
        ~
        \captionsetup[subfigure]{position=b}
        \begin{subfigure}{0.32\textwidth}
                \includegraphics[width=\textwidth]{images/corl/performance_airsim/class_percentage_airsim_photoreal_simu.png}
        \vspace{-5mm}
        \caption{\footnotesize{}\label{fig:classificationspeedReal}}
        \end{subfigure}
        
        \vspace{-5mm}
        %\setcounter{figure}{6}
        \caption{\footnotesize{Mean and standard deviation over 50 experiments in the photo-realistic simulator.
         \textbf{a)}~Comparison of the percentage of targets classified before timeout in environments with 1 to 40 targets taking measurements from the high-level viewpoints.
          ~\textbf{b)}~Classification speed in the photo-realistic environments of 30 targets taking measurements from the high-level viewpoints.~\textbf{c)}~Classification speed in photo-realistic environments of 30 targets with realistic drone dynamics and AirSim's controller.%~\textbf{d)}~Performance comparison of the policy under first order and realistic dynamics.
        }} \label{fig:relperformance}
\end{figure*}
% \vspace{-10mm}

==> sec/limitations.tex <==
\section{Limitations}
Although we have not yet verified our method with a real drone, we expect that the proposed framework will be easily transferable thanks to the realistic low level controller employed in our tests. Our method relies heavily on a key assumption: knowledge of the targets' relative pose. This knowledge could be gained from a different signal than images%
%sensor different than the one used for classification
, e.g., from LiDAR readings, wifi signals, or UWB tags. Recent works address the problem of Searching and Tracking (SAT) multiple targets~\cite{Hsu2021}. However, adding the former to our framework would require to learn to balance SAT with active classification goals. Future work will therefore improve on the robustness of our framework by learning to search, track and classify targets in an unknown map where observations might be partially occluded by static obstacles. We speculate that a generalization to environments with static obstacles could be implemented by either encoding a graphical representation of the global map using a 2D-CNN, or encoding LIDAR measurements using a 1D-CNN. Future work will also relax the assumption that all targets' class information is observable from the same relative orientation. We hope to further generalize our framework to also learn to identify online from where a given classifier can extract useful class information from the targets.
